How to Probe: Simple Yet Effective Techniques for Improving Post-hoc Explanations

Post-hoc importance attribution methods are a popular tool for "explaining" Deep Neural Networks (DNNs) and are inherently based on the assumption that the explanations can be applied independently of how the models were trained. Contrarily, in this work we bring forward empirical evidence that challenges this very notion. Surprisingly, we discover a strong dependency on and demonstrate that the training details of a pre-trained model's classification layer (less than 10 percent of model parameters) play a crucial role, much more than the pre-training scheme itself. This is of high practical relevance: (1) as techniques for pre-training models are becoming increasingly diverse, understanding the interplay between these techniques and attribution methods is critical; (2) it sheds light on an important yet overlooked assumption of post-hoc attribution methods which can drastically impact model explanations and how they are interpreted eventually. With this finding we also present simple yet effective adjustments to the classification layers, that can significantly enhance the quality of model explanations. We validate our findings across several visual pre-training frameworks (fully-supervised, self-supervised, contrastive vision-language training) and analyse how they impact explanations for a wide range of attribution methods on a diverse set of evaluation metrics.

==> sec/0_abstract.tex <==
\begin{abstract}
\vspace{-4mm}

Post-hoc importance attribution methods are a popular tool for ``explaining'' Deep Neural Networks (DNNs). While these methods are inherently designed to be agnostic to how the models were trained, recent studies suggest that the choice of training paradigm can significantly impact explanation quality. \bernt{is it really true that there are studies that show that the choice of training paradigm can significantly impact explanation quality? in the generality of this statement made here - it is diminishing the value of our findings - right? - imho we need should be more specific on what they find and also how our work is different - right?} As techniques for pre-training models are becoming increasingly diverse, understanding the interplay between these techniques and the explanation methods is of high practical importance.
Therefore, we perform an in-depth systematic study of several visual pre-training frameworks (fully-supervised, self-supervised, contrastive vision-language training) and analyse how they impact explanations for a wide range of attribution methods. 
Surprisingly, our experiments suggest that the training details of the models' classification layer play a much more important role than the pre-training scheme and simple yet effective changes in the classification layers can significantly improve the quality of the explanations. 
\blue{\textit{Code to reproduce all experiments: \url{https://anonymous.4open.science/r/how-to-probe-iclr/}} }

\vspace{-2mm}
\end{abstract}


==> sec/figures/bce_vs_ce_quali.tex <==
\begin{figure}[t]
  \begin{center}
    \centering
        \includegraphics[width=0.75\linewidth]{sec/images/bce_vs_ce_qualv2.pdf}
\end{center}
    \vspace{-4mm}
    \caption{
    \textbf{BCE vs.~CE.} The \bcos attributions for a linear probe trained with CE loss (\textbf{bottom row}) leak into nearby cells in the 2x2 GridPG~\cite{codanets} evaluation setting. The attributions for linear probes trained with a BCE loss (\textbf{top row}) are much more localized. This is consistent across pre-training paradigms (SSL and supervised).
    \vspace{-1mm}
    }
   \label{fig:bce_vs_ce_qual}
\end{figure}

==> sec/figures/bce_vs_ce_toy.tex <==
\begin{figure}[t]
  \begin{center}
    \centering
        \includegraphics[width=\linewidth]{sec/images/ce_vs_bce_motivation_toy_v2.pdf}
\end{center}
    \vspace{-4mm}
    \caption{
    \textbf{Due to the shift-invariance of softmax,} {\color[RGB]{234, 52, 38}{positive}} and {\color[RGB]{62, 64, 233}{negative}} attributions do not have a fixed  `meaning' for models trained with the CE loss, which can lead to unintuitive model explanations (left, CE), see also \cref{eq:ce}. Specifically, one can easily define an \textbf{equivalent} linear probe that achieves the same loss under softmax, but yields inverted explanations and negative class logits. To obtain more interpretable post-hoc explanations, we therefore propose to train linear probes with the BCE loss (right).
%
    \bernt{I find this quite confusing - you write something like $g(x_i)[t_i]$ in the figure - but that is not in the equations! neither $g$, nor $x_i$ nor $t_i$????????? -- also in the figure I was overlooking completely that in the last case ``spoonbill'' gets 0\% - which i suppose is the key message? }
    \moritz{Yes, I fully agree, the highlight of the figure should be on 100\% vs.~0\% and the equations should be made consistent}
    \vspace{-1mm}
    }
   \label{fig:bce_vs_ce_toy}
\end{figure}

==> sec/figures/dino_vs_sup.tex <==
\begin{figure}[t]
  \begin{center}
    \centering
        \includegraphics[width=0.75\linewidth]{sec/images/qual_dino_sup_2.pdf}
\end{center}
    \vspace{-4mm}
    \caption{
    {\textbf{SSL vs Supervised}. The \bcos attributions for DINO (\textbf{cols.~2+3}) are visually very similar to supervised models (\textbf{cols.~4+5}), despite being optimized very differently.
    We also see that for \bcos models the improvements in attribution localization for probes trained with BCE loss are consistent for both DINO and supervised models. These results are further consistent across for \moco and \byol, see supplement.% for more qualitative results.
    }
    \vspace{-1mm}
    }
   \label{fig:dino_vs_sup}
\end{figure}

==> sec/figures/mlp_ablation.tex <==
\begin{subfigure}[c]{\linewidth}
\centering
\begin{center}
    \centering
    \includegraphics[width=\linewidth]{sec/images/bcos_mlp_in1k_100_flat.pdf}
\end{center}
\vspace{-4mm}
    \caption{
    \vspace{3mm}
    }
    \label{fig:mlp_ablation}
% \end{figure*}
\end{subfigure}


==> sec/figures/mlp_ablation_coco.tex <==
\begin{subfigure}[c]{\linewidth}
\begin{center}
    \centering
    \includegraphics[width=\linewidth]{sec/images/bcos_mlp_coco_100_flat.pdf}
\end{center}
\vspace{-4mm}
    \caption{
    }
    \label{fig:coco_mlp_ablation}
% \end{figure*}
\end{subfigure}


==> sec/tables/bce_vs_ce_loc_delta.tex <==
\begin{table}[t]
\caption{\textbf{CE vs.~BCE.} Accuracy and \gridpg scores for \lrp for conventional and \bcos explanations for \bcos models. We observe a consistent, albeit small drop in accuracy when training linear probes via BCE. Importantly, however, BCE leads significantly improves object localization as measured by the \gridpg score, despite explanations and frozen features being the same for every given pre-training method. \sid{what additional utility does this add compared to figure 4?}
\vspace{-.2cm}
}
{
\fontsize{7pt}{9pt}\selectfont
\centering
% {l@{\hskip2pt}c@{\hskip8pt}c@{\hskip20pt}c@{\hskip8pt}c@{\hskip20pt}c@{\hskip8pt}c@{\hskip2pt}}
\begin{tabular}
{l@{\hskip10pt}cccc@{\hskip10pt}cccc@{\hskip10pt}cccc@{\hskip10pt}ccc}
% \fontsize{5pt}{5pt}\selectfont
 \toprule
& \multicolumn{7}{c}{\bf \bcos Models} &&  \multicolumn{7}{c}{\bf Conventional Models \\ %[1em]
 \midrule
 %\hline
 \textbf{Method} &\multicolumn{3}{c}{\textbf{Accuracy (\%)}} && \multicolumn{3}{c}{\textbf{\gridpg (\%)}}&&\multicolumn{3}{c}{\textbf{Accuracy (\%)}} && \multicolumn{3}{c}{\textbf{\gridpg (\%)}}\\ %[.5em]
 \midrule
 %\hline
 & CE& BCE & $\Delta$ && CE&BCE& $\;\Delta$&& CE& BCE & $\Delta$ && CE&BCE& $\;\Delta$ \\
{\moco}& 66.3&  {  63.2} &{ \color{red} \makebox[.15cm][r]{-}3.1}  &&48.0 & 81.0&{ \color{teal} +33.0} && 67.5&  {  64.5} &{ \color{red} \makebox[.15cm][r]{-}3.0} && 50.0 & 80.0 &{ \color{teal} +30.0} \\
 {\byol}& 68.3 &  {  68.1} &{ \color{red} \makebox[.15cm][r]{-}0.2}  &&43.0 & 71.0 &{ \color{teal} +28.0}&& 70.1&  {  69.3} &{ \color{red} \makebox[.15cm][r]{-}0.8} &&48.0 & 66.0 &{ \color{teal} +18.0} \\
 {\dino}& 68.2&  {  67.5} &{ \color{red} \makebox[.15cm][r]{-}0.7} & &43.0 &80.0 &{ \color{teal} +37.0}&& 71.2&  {  70.6} &{ \color{red} \makebox[.15cm][r]{-}0.6} &&52.0 & 92.0&{ \color{teal} +40.0} \\
CLIP& - &  - & -  && -  & - & - && 72.6&  {72.9} &{ \color{teal} +0.3} &&19.0 & 51.0&{ \color{teal} +32.0}\\
 {Supervised}&74.5 &  {  75.9} &{ \color{teal} +1.4 }  &&25.0 & 92.0&{ \color{teal} +67.0}&&76.5&  {  74.3} &{ \color{red} \makebox[.15cm][r]{-}2.2} && 59.0 & 64.0&{ \color{teal} +\phantom{3}5.0}\\
 \bottomrule
\end{tabular}
}
\label{tab:bce_vs_loc}
\end{table}

==> sec/tables/imagenet_linear_classification_v2.tex <==
\begin{table}[t]
    \centering
    %\resizebox{\linewidth}{!}{
    \small
    \caption{
    \textbf{Linear probe accuracy on \imagenet} for conventional (RN50) and \bcos (B-RN50) ResNet-50 models trained via \moco, \byol, and \dino; results for the respective supervised models shown for reference. We find \bcos models to achieve similar performance via SSL probing as their conventional counterparts, with similar performance drops as for supervised training.
    } 
    \label{tab:image_net_top1}
    \vspace{-3mm}
    \begin{tabular}{lcc}
    % \toprule
	  & \multicolumn{2}{c}{\textbf{Accuracy (\%)}} \\[.25em]
 \bf Method&{\small B-RN50}&{\small RN50}\\%[.5em]
    \midrule
    % \cmidrule(lr){1-1}
    % \cmidrule(lr){2-2}
    % \cmidrule(lr){3-4}
    \multirow{1}{*}{MoCov2~\cite{mocov2}} & 66.3 & 67.5 \\
    %\hline

    \multirow{1}{*}{BYOL~\cite{byol}} & 68.3 & 70.1 \\
    %\hline    
    \multirow{1}{*}{DINO~\cite{dino}} & 68.2 & 71.2\\
    %\hline
    \multirow{1}{*}{Supervised} & 74.5 & 76.5 \\
     \bottomrule
    \end{tabular}
    %}
    %\vspace{-2mm}

    % \vspace{-12pt}
\end{table}
